Evaluating Online Continual Learning with CALM

Online Continual Learning (OCL) studies learning over a continuous data stream without observing any single example more than once, a setting that is closer to the experience of humans and systems that must learn "on-the-wild". Yet, commonly available benchmarks are far from these real-world conditions, because they explicitly signal different tasks, lack latent similarity structure or assume temporal independence between different examples. Here, we propose a new benchmark for OCL based on language modelling in which input alternates between different languages and domains without any explicit delimitation. Additionally, we propose new metrics to study catastrophic forgetting in this setting and evaluate multiple baseline models based on compositions of experts. Finally, we introduce a simple gating technique that learns the latent similarities between different inputs, improving the performance of a Products of Experts model.

==> growing_models.tex <==
\section{Growing models} 

%As mentioned in the previous section, 
Growth in neural networks has been explored with different perspectives.
Here, we present a discussion of the possible avenues for developing neural
networks with unbounded memory.

\begin{enumerate}
\item Growth of layers: Early work on Neural Networks used this method to
reduce the amount of computational complexity or for escaping local minima~\citep{fahlman1990cascade,hirose1991back}.
The goal, back then, was using the smallest possible number of hidden units.
Here, instead, we are interested in allowing neural networks to grow for endowing
them with larger memory capacity. In this sense, this strategy seems limited
because all units remain fully connected at all time, forcing the network to
access all memories simultaneously.

%can be achieved by adding neurons to hidden layers. How should
%the weights be initialized? What are the problems: still fully connected, grows
%but accesses all the parameters - does not seem very practical. On top of it,
%empirical results are not very promising (we could do some experiment of this sort).

\item Growth of architecture: A different type of growth could be the one
dictated by a different model that decides the characteristics of the learning
system, including how many units to put in it. Neural architecture
search~\citep{elsken2018neural}
and, particularly, neuro-evolution~\citep{Stanley2019} provide good examples of this.
Note, however, that this type of growth is different from the main problem
that we are dealing with here, in which a model needs to be able to extend \emph{itself}.

%\item Learned, structured growth: stack-RNNs where the number of neurons can increase
%based on the given instance of a problem, assuming the model has been
%previously correctly trained. The model itself learns how much computational resources
%is used, but so far only this has been demonstrated only on toy problems like
%sequence memorization. Stack-RNNs are also unable to quickly recover "memories"
%from distant past (ie. would have to cycle through the whole stack, step-by-step).
\item Learned, structured growth: Models, like the Stack-RNNs~\cite{joulin2015inferring} 
permit the model to create new units, which are placed on a stack data structure,
allowing it thus to have a flexible memory to process different problem instances
of varying sizes. The model itself learns how many computational resources
to use, but so far this has been demonstrated only on toy problems like
sequence memorization. Moreover, Stack-RNNs are also unable to quickly recover
``memories'' from distant past because it would imply cycling through the whole
stack.

\item Sparse growth: This is the strategy that we focus on in this paper. 
The network is grown by blocks or modules. One potential drawback with this 
strategy is the linear increase of time complexity as the network grows. To 
prevent this, here we simply limit the maximum number of modules that are kept
alive at any given time. Other, more sophisticated, options could employ a
Hierarchical Softmax~\citep{goodman2001classes} operation over the modules or
Winner-Takes-All types of rules~\citep{srivastava2013compete}, essentially
searching for just the right memories to answer the current situation.
\end{enumerate}



% I think this was just repeated:
% \textbf{Growing models}
% 
% Here, we should describe some of the existing models of growth in neural networks,
% and add our ideas into the picture. The story could go as follows:
% 
% 1) Growth of layers: can be achieved by adding neurons to hidden layers. How should
% the weights be initialized? What are the problems: still fully connected, grows
% but accesses all the parameters - does not seem very practical. On top of it,
% empirical results are not very promising (we could do some experiment of this sort).
% 
% 2) Growth of architecture: architecture search could be disccussed here. We can have
% a meta-learning technique where we evaluate different architectures for a given
% problem, and choose the best. This can result in quite complex architectures with
% many hidden layers that are non-trivially connected. Still the same limitations
% as in 1)
% 
% 3) Learned, structured growth: stack-RNNs where the number of neurons can increase
% based on the given instance of a problem, assuming the model has been
% previously correctly trained. The model itself learns how much computational resources
% is used, but so far only this has been demonstrated only on toy problems like
% sequence memorization. Stack-RNNs are also unable to quickly recover "memories"
% from distant past (ie. would have to cycle through the whole stack, step-by-step).
% 
% 4) Sparse growth: what we will focus on in this paper - we grow the NN by blocks, and
% we discuss mechanisms how to avoid linearly increasing time complexity (simple hack
% is to have a fixed number of the "clones", another should be to have something like
% a hierarchical softmax over the clones).

